Chemo-kinematics of the $Gaia$ RR Lyrae: the halo and the disc

We present the results of a multi-component kinematic model of a large sample of RR Lyrae detected by $Gaia$. By imposing a four-fold symmetry and employing $Gaia$ proper motions, we are able to infer the behaviour of the velocity ellipsoid between $\approx3$ and $\approx30$ kpc from the centre of the Galaxy. We detect the presence of two distinct components: a dominant non-rotating halo-like population and a much smaller rotating disc-like population. We demonstrate that the halo RR Lyrae can be described as a superposition of an isotropic and radially-biased parts. The radially-biased portion of the halo is characterised by a high orbital anisotropy $\beta\approx0.9$ and contributes between 50\% and 80\% of the halo RR Lyrae at $5<R$(kpc)$<25$. In line with previous studies, we interpret this high-$\beta$ component as the debris cloud of the ancient massive merger also known as the $Gaia$ Sausage (GS) whose orbital extrema we constrain. The lightcurve properties of the RR Lyrae support the kinematic decomposition: the GS stars are more metal-rich and boast higher fractions of Oosterhoff Type 1 and high amplitude short period (HASP) variables compared to the isotropic halo component. The metallicity/HASP maps reveal that the inner 10 kpc of the halo is likely inhabited by the RR Lyrae born in-situ. The mean azimuthal speed and the velocity dispersion of the disc RR Lyrae out to $R\approx30$ kpc are consistent with the behaviour of a young and metal-rich thin disc stellar population.

==> include/disc.tex <==
\section{The disc of RRLyrae stars} \label{sec:disc}


Result about the disc

remember this paper \url{https://arxiv.org/pdf/1810.09466.pdf}



\begin{figure*}
\centering
\centerline{\includegraphics[width=1.0\textwidth]{image_new/Vphi_disp_disc}}
\caption[]{Rotational velocity and velocity dispersion (assumed isotropic) obtained for the sample of rotating stars (see Sec.). Along the y-axis, the points indicate the median of the a-posteriori distribution of the azimuthal velocity, while the errorbars indicate its 16th and 84th percentile.  Along the x-axis, the points indicate the median of the cylindrical radial distribution, while the errorbars indicate the median value of the errors on the cylindrical radius of the stars in the given bin. 
 The black dashed lines indicate a  5 kpc radius that is roughly the region where the presence of the bar could be important. The vertical dashed line in the first panel indicates $V_\phi=230 \ \kms$. The grey bands shows the $1 \sigma$  and $2\sigma$  interval from a Gaussian Process interpolation. The blue band show the 1$\sigma$ interval of the posterior obtained using the SA ($SOS$+$ASSASN$) catalogue (see text). The large errors for the SA results around 12 kpc are due to a bin where most of stars has been classified as background. The magenta line in the left-hand panel shows the rotational velocity found by \cite{Ablimit20} using a sample of Cepheids. The blue and orange lines in the right-hand panel show the fit of the Galactic (vertical) velocity dispersion by \cite{Sharma20} assuming [Fe/H]=$-1.0$ (see Fig.\ \ref{fig:disc_halo_compare}), $z=0.5\ \kpc$ and stellar age $t=3.5 \ \Gyr$ (orange line) and $t=10 \ \Gyr$ (blue line), see text for further information.}
\label{fig:disc_vrot}
\end{figure*}



\begin{figure*}
\centering
\centerline{\includegraphics[width=1.0\textwidth]{image_new/halo_disc_props}}
\caption[]{Distribution of  properties for  a subsample of RRL stars in the halo  (red, see Sec. ???)  and disc sample (blue, see Sec. ???) of the ??? catalogue (see Sec. ???). From top-left to bottom-right the panels show the metallicity estimated in this work (see Sec.), the period of the RRab stars, the light curve phase difference $\Phi_\mathrm{31,G}$ (see Sec. xx), the metallicity from \gaia SOS, the first overtone period of the RRc stars and the light curve amplitude in the $G$ band. The vertical dashed lines indicate the value of the median of the distributions. Only stars that have an estimate of both period and  light curve phase difference  have been considered for this plot ($24598$ and $1146$  stars for the halo and disc sample, respectively.).}
\label{fig:disc_halo_compare}
\end{figure*}

\begin{figure*}
\centering
\centerline{\includegraphics[width=0.8\textwidth]{image_new/sharma_plot.pdf}}
\caption[]{}
\label{fig:sharma_paper}
\end{figure*}



\begin{comment}

\begin{figure*}
\centering
\centerline{\includegraphics[width=1.0\textwidth]{image/Vphi_disp_disc}}
\caption[]{Rotational velocity and velocity dispersion (radial and vertical) obtained for the sample of rotating stars ($f^{MAP}_{rot}>0.7$, $f^{16th}_{rot}>0.5$, $|z|<3.8 \ \mathrm{kpc}$, Voronoi binned with S/N target 7). The grey dashed lines indicate the 5 kpc radius that is roughly the region where the presence of the bar can be important.}
\label{fig:disc_vrot}
\end{figure*}


\begin{figure*}
\centering
\centerline{\includegraphics[width=1.0\textwidth]{image/Vphi_disc_combined.pdf}}
\caption[]{Results of the two-component disc fit. In the model we call thin (thick) component the one with prior on the rotational velocity bounded between 180 km/s (0 km/s) and 300 km/s (150 km/s). Left: Rotational velocity, the bands show the regions bounded by the prior distribution. Right: fraction of thin component, the blue bands show the 1-$\sigma$  confidence interval of a GP process fitting including a component for the intrinsic scatter. It is evident that instead of having the mix of two components we have two regimes dominated by a thick-disc and a thin-disc like kinematic. The grey dashed lines indicate the 5 kpc radius that is roughly the region where the presence of the bar can be important. The transition among the two kinematic regimes seems to happen around this radius.}
\label{fig:disc_vrot_2comp}
\end{figure*}


\begin{figure*}
\centering
\centerline{\includegraphics[width=1.0\textwidth]{image/SOS_RRab_halo_disc_metallicity.pdf}}
\caption[]{}
\label{fig:disc_halo_metallicity}
\end{figure*}


\begin{figure*}
\centering
\centerline{\includegraphics[width=0.7\textwidth]{image/disc_metal.pdf}}
\caption[]{Metallicity vs circular radius. The blue points indicate the metallicity (from Lamost) of thin disc stars ($q_{MAP}>0.5$), the green points of the thick disc stars ($q_{MAP}>0.5$) (from SOS sample).  The shaded contours show the metallicity of the  thin disc (blue), thick disc (green) as measured in SOS, while the red contours show the metallicity of the halo stars (SOSxASSAN) measured in Lamost. THe contours levels are 5,20,40,50,100.}
\label{fig:disc_metal}
\end{figure*}

\end{comment}

==> include/halo.tex <==
\section{halo} \label{sec:halo}

Results about the halo

\begin{figure*}
\centering
\centerline{\includegraphics[width=0.8\textwidth]{image_new/combo_halo_cat2_radial}}
\caption[]{Results of the anisotropic/radial component of the halo: relative fraction of the radial component over the total (top panels), anisotropy (middle panels) and the position of the peak of the double-horn profile assumed for the distribution of the radial velocity (see Sec. xxx, bottom panels). 
 The left-hand panels show the results of the 1D spherical fit (see Sec. xxx): along the y-axis, the large-yellow points indicate the median of the a-posteriori distribution of the given property, while the errorbars indicate its 16th and 84th percentile; the small-red points show the Maximum-a-Posteriori (MAP) of the posteriors;  along the x-axis, the points indicate the median of the spherical radial distribution, while the errorbars indicate the median value of the errors on the radius of the stars in the given bins; the vertical dashed line in the first panel indicates $V_\phi=230 \ \kms$; the grey bands show the $1 \sigma$  and $2\sigma$  interval from a Gaussian Process (GP) interpolation. The GP interpolator has been fitted to a symmetrised version of the data points: the y-values are the middle points between the 16th and 84th percentile, while the y-errors are half of the 16th-84th percentile distance; the blue band show the 1$\sigma$ interval of the posterior obtained using the SA ($SOS$+$ASSASN$) catalogue (see text). The right-hand panels show the results of the 2D cylindrical fit (see Sec. xxx): the circular lines indicate the spherical radii 5,8,10,15,20,25 kpc.
 In some cases the Median and MAP estimates show large differences, in that cases the posteriors show a significant bimodal distribution and the median is close to the minimum that has been sampled more. In that cases, the error-bars are not showing classical Gaussian-like 1$\sigma$ errors but rather the distance between the two minima sampled by the MCMC. 
 Despite the large uncertainties a clear trend appears after 15/18 kpc: if we consider the MAP the fraction of the radial component remains high but $L_\mathrm{r}$ drops to 0; if we consider the Median $L_\mathrm{r}\sim50 \ \kms$, but the fraction drops to small values. Therefore, both the MAP and Median indicate a transition between the strong radially anisotropic component and something else at $r>15$ kpc.}
\label{fig:halo_comb}
\end{figure*}


\begin{figure*}
\centering
\centerline{\includegraphics[width=1.0\textwidth]{image_new/combo_halo_Vphi_red}}
\caption[]{Same as Fig. \ref{fig:halo_comb} but for the azimuthal velocity for the anisotropic/radial (left-hand panel) and the isotropic (right-hand panel)  components.}
\label{fig:halo_comb_vphi}
\end{figure*}

\begin{figure*}
\centering
\centerline{\includegraphics[width=1.0\textwidth]{image_new/1comp_combo_red}}
\caption[]{Same as Fig. \ref{fig:halo_comb} but for the anisotropy (left-hand panel) and the azimuthal velocity (right-hand panel) estimated in the 1-component fit of the halo catalogue (see Sec. xxx).}
\label{fig:halo_comb_1comp}
\end{figure*}


\begin{figure*}
\centering
\centerline{\includegraphics[width=1.0\textwidth]{image_new/combs_feh.pdf}}
\caption[]{Cylindrical maps showing the median of the metallicity distribution estimated in this work (top panels) and in the SOS catalogue (bottom panels). The left-hand panels show the metallicity map considering the stars belonging to the radial halo component ($23,734$ stars) while the middle panels shows the stars belonging to the isotropic halo component ($7,767$ stars). The right-hand panels show the difference between the radial and isotropic maps. The stars used to make in this map are from a subsample of the halo catalogue (see Sec.) obtained considering only the stars beloging to the SOS catalogue and with a a-posteriori MAP likelihood to belong to the radial or isotropic component larger than 0.7. The Voronoi-tesselation has been obtained using the isotropic halo component with a target SN equals to 10. The bins in which the number of stars is lower than 50 are excluded in the maps (see e.g. the white bins in the left-hand and right-hand panels).}
\label{fig:halo_comb_met}
\end{figure*}

\begin{figure*}
\centering
\centerline{\includegraphics[width=1.0\textwidth]{image_new/combo_halo_fHASP.pdf}}
\caption[]{Same as Fig. \ref{fig:halo_comb_met} but for the RRL Type 1  (top panels) and the RRL HASP (bottom panel) fraction. See Sec.xx and \cite{BelokurovHASP}.}
\label{fig:halo_comb_fHASP}
\end{figure*}




\begin{comment}
\subsection{one-component model}

\begin{figure*}
\centering
\centerline{\includegraphics[width=1.0\textwidth]{image/summary_1comp_halo.pdf}}
\caption[]{}
\label{fig:halo_2comp_summary}
\end{figure*}


\subsection{two-component model}

\begin{figure*}
\centering
\centerline{\includegraphics[width=1.0\textwidth]{image/summary_2comp_halo.pdf}}
\caption[]{}
\label{fig:halo_2comp_summary}
\end{figure*}


\begin{figure*}
\centering
\centerline{\includegraphics[width=1.0\textwidth]{image/summary_vrot_2comp_halo.pdf}}
\caption[]{}
\label{fig:halo_vrot_2comp_summary}
\end{figure*}


\begin{figure*}
\centering
\centerline{\includegraphics[width=0.8\textwidth]{image/halo_2comp_metallicity.pdf}}
\caption[]{Comparison of the metallicity distribution (from SOS, left; from Lamost, right) for the 2 components of the halo fit (SOSxASSASN). Top panels: stars within 10 kpc, bottom panels: stars with radius larger than 10 kpc. We considered only stars with $q_MAP>0.7$ for the specific component.}
\label{fig:halo_vrot_2comp_summary}
\end{figure*}

\begin{figure*}
\centering
\centerline{\includegraphics[width=0.8\textwidth]{image/met_rad_p_2comp_halo.pdf}}
\caption[]{Metallicity vs spherical radius (left) and period (right) for the 2 components of the halo fit (SOSxASSASN).}
\label{fig:halo_vrot_2comp_summary}
\end{figure*}
\end{comment}


==> include/kinematicSeparation.tex <==
\section{Kinematic separation} \label{sec:kseparation}

Figure XXX shows the distribution of the posterior probability of
belonging to the non-rotating (halo) component for the stars in our
sample. The distribution has three distinct parts: the main peak
around $q=1$ -- these are the RR Lyrae that do not exhibit any
significant rotation and thus can be assigned to the halo; a smaller
bump around $q=0$ contributed by the stars with disc-like kinematics;
finally, in between the two peaks, there is a flat, low-amplitude
component composed of stars that do not fall squarely in one of the
two groups. Setting the third, undetermined group aside, we focus on
the stars that can be classified as halo or disc with certainty. We
apply the following criteria using the posterior probabilities
calculated as described above.

%
\begin{equation}
XXX=YYY
\end{equation}
%

Of the total 72973 RR Lyrae in our sample, 49914 (or $\sim68\%$) are
classified as halo, 3126 (or $\sim4\%$) as disc; while the remaining
20353 ($\sim28\%$) are unclassified. Figure~\ref{fig:maps} shows the
distribution of the whole sample and the three groups on sky in
Galactic coordinates (top row) and in cylindrical $R, |z|$ (bottom
row). The halo stars (second column)) span a wide range of Galactic
latitudes but mostly reside in a centrally concentrated, flattened
structure limited by $R<30$ kpc and $|z|<20$ kpc. Strikingly, the
rotating component (third column) is mostly limited to
$|b|<20^{\circ}$ and $|z|<5$ kpc but extends to $R\sim30$
kpc. Finally, the shape of the unclassified portion of our sample
(fourth column) resembles that of the halo, albeit more concentrated
to the centre: most of the stars are at $R<10$ kpc and $|z|<5$
kpc. Additionally, at higher $|z|, $there are several lumps and lobes
likely corresponding the parts of the Virgo Overdensity and the
Hercules Aquila Cloud
\citep[e.g.][]{Vivas2001,Vivas2006,HAC2007,Juric2008,Simion2014,Simion2019}.

Figure~\ref{fig:disc_vrot} presents the maps of the kinematic
properties of the two principle components, the halo and the disc in
cylindrical $R$ and $|z|$. The two rows give the same information, but
the bottom row shows the results of the 2-component fit only if there
is a significant improvement as indicated by the Bayesian Information
Criterion $\Delta {\rm BIC}>10$, otherwise it reverts to the results
of a single-component fit. The first column shows the map of the
fractional contribution of the RR Lyrae disc. While there are some
hints of rotating parts of the halo at high $|z|$ in the op panel, as
demonstrated by the bottom panel, these are not significant
enough. The bulk of the rotating component sits at $|z|<5$ kpc across
a wide raneg of $R$, and closer to the Sun its vertical extent is
clearly limited to a couple of kpc at most. The second column presents
the map of the azimuthal velocity $v_{\phi}$ as a function of $R$ and
$|z|$. Again, some Voronoi cells at high $|z|$ may have the kinematics
consistent with a slow rotation, however $\Delta{\rm BIC}$ criterion
renders them not significant enough. Therefore, in the bottom row,
these high $|z|$ cells are empty and the bulk of the $v_{\phi}$ map is
limited to low vertical heights where the rotation velocity is in
excess of $v_{\phi}>200$ kms$^{-1}$ across the entire range of
$R$. Finally, the third column displays the behaviour of the halo
velocity anisotropy $\beta$ as mapped by RR Lyrae. Except a small
region near the centre of the Milky Way and a few cells at high $|z|$
where the motion appears nearly isotropic, the rest of the halo
exhibits strong radial anisotropy with $0.5<\beta<0.9$.

%
\begin{figure*}
\centering
\centerline{\includegraphics[width=1.2\textwidth]{image_new/halo_disc_combo_cat2.pdf}}
\caption[]{Cylindrical maps of some MAP results of the double
  component fit for RRL in the xxx sample. The panels in the first row
  show the results of the 2-component model fit. The panels in the
  second row show the mixed 1 and 2 component results (results from
  the 2-component fit if $\Delta \mathrm{BIC}>10$, otherwise from the
  1-component fit, see text).  The panels in the first column show the
  fraction of the rotating component, in the second column the
  azimuthal velocity of the disc component and in the third column the
  anisotropy of the halo component.}
\label{fig:disc_vrot}
\end{figure*}
%


==> include/method.tex <==
\section{method} \label{sec:method}

The aim of this work is to study the kinematics of the RRL stars 
in the \gaia dataset. The  is however limited by the lack  line-of-sight velocity measurement  for most of the stars in our final catalogue, indeed only 266  over more than $70,000$ stars have \gaia radial velocity. Cross-matching with other catalogue as RAVE (cit), APOGEE (cit) and LAMOST (cit)  will reduce both the radial extension and/or the sky coverage of the \gaia catalogue.   {\giu Estimate the number of stars in common with these cats..}.  Moreover, the periodic radial  expansion/contraction of the stellar layers in RRLs, if not taken into account,  can bias the  radial velocity measurements up to $40-70\ \kms$ \cite[see e.g.][]{Liu91,Drake2013}. 
The large sky coverage of our dataset let us also to extended the kinematic analysis from the stellar halo to the relatively less explored (considering the RRL populations)  stellar disc.
The estimate of the full 3D velocity information on a star by star basis is not possible without the knowledge of the line-of-sight velocity, however since stars at different position in the Sky and distance have different projections on the 3D Galactic velocity space, it is possible to estimate the velocity moments (mean values and standard deviation) of the intrinsic 3D velocity ellipsoid   from the proper motions of a group of stars taken together \cite[see e.g.][]{Dehnen98,Schonrich12,Schonrich18,Wegg19}. 

\subsection{Kinematic fit}

For the purpose of our work we decide to implement a velocity moments method following and the extending the method by \cite[][, \WG hereafter]{Wegg19}.  In this section we briefly summarise the method, further  details can be found in the original \WG paper. 
The basic assumption of the the method is that the intrinsic velocity distribution of stars in a given Galactic volume and in given Galactocentric coordinates (e.g. Spherical or Cylindrical) is a multivariate normal $f\left(\bm{V}\right)=\mathcal{N} \left( \bar{\bm{V}},\Sigma \right)$, where $\bar{\bm{V}}$ is the Gaussian centroid and $\Sigma$ is the covariance matrix or velocity dispersion tensor. This distribution can be projected on the sky coordinates $\bm{V}_\mathrm{sky}=(V_\mathrm{los}, V_\ell, V_b)$ simply through the rotation matrix $\mathbf{R}$ (different for each sky position) satisfying  $\bm{V}_\mathrm{sky}=\mathbf{R}\bm{V}$. The projected distribution is still a Gaussian therefore it can be easily analytically marginalised over the unknown term $V_\mathrm{los}$. Finally, the likelihood for a given star located at given distance and position on the sky to have velocities $\bm{V}_\mathrm{\perp}=(V_\ell, V_b)$ is given by the two dimensional Multivariate Gaussian
\begin{equation}
\mathcal{L} = \mathcal{N}\left( \bar{\bm{V}}_\mathrm{\perp}, \Lambda_\perp + \mathbf{S} \right),
\label{eq:lk}
\end{equation}
where 
\begin{itemize}
    \item $\bar{\bm{V}}_\mathrm{\perp} = \mathbf{R}_\perp  \bar{\bm{V}}$ and $\mathbf{R}_\perp$ is the rotation matrix $\mathbf{R}$ without the 1st row related to the los velocity ($2\times3$ matrix, see Appendix \ref{appendix:rotation_matrix}); 
    \item $\Lambda_\perp$ is the projected covariance matrix  $\Lambda=\mathbf{R}\mathbf{\Sigma}\mathbf{R}^\intercal$ without the 1st row and the 1st column related to the los velocity  ($2\times2$ matrix);
    \item $\mathbf{S}$ is a 2x2 matrix of the $V_\ell, V_b$ measurement covariance (see Sec.\ \ref{sec:dist_estimate}).
\end{itemize}
In order to estimate the velocity moments, we consider the total likelihood as the product of the likelihoods (Eq.\ \ref{eq:lk}) of all the stars in a given Galactic volume bin. The method described so far follows, point by point,  what has been done in \WG. We add a further generalisation considering the intrinsic velocity distribution  as a composition of multiple multivariate normal distributions. Therefore the likelihood for a single star becomes
\begin{equation}
\mathcal{L}_\mathrm{multi} = \sum_i \omega_i \mathcal{N}\left( \bar{\bm{V}}_{i,\mathrm{\perp}}, \Lambda_{i,\perp} + \mathbf{S}_i \right)=\sum_i \omega_i \mathcal{L}_i,
\label{eq:lkmulti}
\end{equation}
where the component weights $\omega$ sum up to 1.  Using Eq.\ \ref{eq:lkmulti} we can apply a Gaussian Mixture Model to the intrinsic distribution fitting only the distribution of observed velocities.  Starting form Eq.\ \ref{eq:lkmulti} it is possible to define, for each star, the a-posterior likelihood  to belong to the $i$th component as 
\begin{equation}
q_i = \frac{\omega_i \mathcal{L}_i}{\mathcal{L}_\mathrm{multi}}. 
\label{eq:lkmulti}
\end{equation}
The stochastic variables $q$ (and their uncertainties)  let us to decompose the stars in different kinematic populations using a quantitative ``metric". 
For a given sample of stars (see Sec.\ \ref{sec:binning}), we retrieve the  properties ($\bm{V}, \mathbf{\Sigma}$) (3+6 parameters) of the kinematic components and their weights adopting a Monte Carlo Markov Chain (MCMC) to sample the  posteriors generate by the product of all the likelihoods defined in Eq.\ \ref{eq:lkmulti}.  In practice, the posterior distributions have been sampled using the affine-invariant ensemble sampled MCMC method implemented in the \texttt{Python} module \texttt{emcee}. We used 50 walkers evolved for 50000 steps after 5000 burn-in steps.  
In the next sections, we exploit this method to separate the RRL stars in our sample in two kinematic components and study their properties: a non or weakly rotating halo-like population and  population with a significant rotation. Moreover, we use again the Gaussian decomposition to separate kinematically the halo in an anisotropic or isotropic population. The chosen intrinsic coordinate system (Spherical or Cylindrical), the number of Gaussian components and the prior distribution of their parameters are described in details in the next sections (see Sec.\ \ref{sec:kseparation}, Sec.\ \ref{sec:halo} and Sec.\ \ref{sec:disc})

\subsection{Binning strategy} \label{sec:binning}
Each of our kinematic fitting analysis is applied to stars grouped in
Galactic bins. In each of those bins the intrinsic distribution of the
velocities is constant. The basic assumptions are axysimmetry and
symmetry with respect to the Galactic plane, in practice we group
stars in the Galactic $R,|z|$ plane. In order to have approximately
the same Poission signal-to-noise ratio ($\sqrt{N_\mathrm{stars}}$) in
each bin we make a Voronoi tessellation of the plane making use of the
\texttt{vorbin} \texttt{Python} package
\citep{Cappellari03}\footnote{\url{https://www-astro.physics.ox.ac.uk/~mxc/software/\#binning}}. When,
we analyse the stars belonging to the halo (Sec.\ \ref{sec:halo}) we
assume a full spherical symmetry binning the stars in Galactic $r$. In
that case, we select the bin edges so that each bin contains
$N_\mathrm{stars}$ stars. If the outermost bin remains with a number
of stars lower than $N_\mathrm{stars}$, we merge it with the adjacent
bin.  In the rest of the paper, we identify the coordinates of a given
bin ($R,|z|$ or $r$) as the median of the of the coordinate of each
stars in the bin, we associate to these values an error that is median
of the correspondent errors of the stars.  The errors on $V_\ell$ and
$V_b$ already take into account the errors on distance
(Sec.\ \ref{sec:dist_estimate}), but we do not take account errors on
$R$,$|z|$ and $r$ in the kinematic fit. In practice, we do not allow a
stars to belong to more than one bin even if this is consistent with
the errors on the Galactic coordinates. This choice do not represent a
serious issue in our analysis, but especially at large radii, where
the errors are larger, the kinematic results of adjacent bin are
likely correlated.


==> include/models.tex <==
\section{Separation of disc and halo}

\begin{figure*}
\centering
\centerline{\includegraphics[width=1.0\textwidth]{image/fd_paper_ASSASN.pdf}}
\caption[]{Fraction of stars belonging to the rotating component. The three panels shows from the left to the right the 16th, 50th and 84th percentile of the posterior distribution.}
\label{fig:dynbestfit}
\end{figure*}



\begin{table}
\begin{tabular}{l|cc}
\hline
\multicolumn{1}{c|}{}                       & SOS (RRab) & SOSxASSASN (RRab) \\ \hline
$f^{MAP}_{rot}>0.5$                         &   6126 (10\%)      &      1662 (10\%)             \\
$f^{50th}_{rot}>0.5$                        &    6337 (10\%) &     1568 (10\%)               \\
$f^{MAP}_{rot}>0.7$ \& $f^{16th}_{rot}>0.5$ &   2742 (4\%)         &     671 (4\%)             \\
$f^{MAP}_{rot}>0.9$ \& $f^{16th}_{rot}>0.5$ &   608 (1\%)         &     155 (1\%)             \\ 
$f^{MAP}_{h}>0.7$ \& $f^{16th}_{h}>0.5$ &   50062 (81\%)         &     13883 (82\%)             \\
$f^{MAP}_{h}>0.9$ \& $f^{16th}_{h}>0.5$ &   48905 (78\%)         &     13309 (79\%)             \\ \hline
\end{tabular}
\end{table}




==> include/rrlage.tex <==
\section{RRL age}

\begin{figure*}
\centering
\centerline{\includegraphics[width=0.9\textwidth]{image/RRLyrae_Minage.pdf}}
\caption[]{Courtesy of A. Savino \cite{savino15}}
\label{fig:dynbestfit}
\end{figure*}



